Evaluating the Diversity, Equity and Inclusion of NLP Technology: A Case Study for Indian Languages

In order for NLP technology to be widely applicable, fair, and useful, it needs to serve a diverse set of speakers across the world's languages, be equitable, i.e., not unduly biased towards any particular language, and be inclusive of all users, particularly in low-resource settings where compute constraints are common. In this paper, we propose an evaluation paradigm that assesses NLP technologies across all three dimensions. While diversity and inclusion have received attention in recent literature, equity is currently unexplored. We propose to address this gap using the Gini coefficient, a well-established metric used for estimating societal wealth inequality. Using our paradigm, we highlight the distressed state of current technologies for Indian (IN) languages (a linguistically large and diverse set, with a varied speaker population), across all three dimensions. To improve upon these metrics, we demonstrate the importance of region-specific choices in model building and dataset creation, and more importantly, propose a novel, generalisable approach to optimal resource allocation during fine-tuning. Finally, we discuss steps to mitigate these biases and encourage the community to employ multi-faceted evaluation when building linguistically diverse and equitable technologies.

==> deprecated.tex <==
\section{Introduction}
The last years saw the development of both a large number of monolingual language models pre-trained in different languages as well as of massively multilingual language models (MMLMs) trained on around 100 languages. While monolingual models often achieve good performance for a given language, they cannot easily be applied to other languages. MMLMs, on the other hand, enable transfer between languages, at the cost of reduced performance on under-represented languages. \\ In order to enable NLP for under-represented languages, we argue for the development of a third category of models, language family-specific models that cover a range of genetically related languages. We illustrate the benefits of such models and aim to provide general recommendations regarding the pre-training data, tokenization, fine-tuning, and evaluation of such models in practice.

\seb{For the title, how about something that emphasizes the language family direction? Maybe something like ``Towards language family-specific language models: A study on Indian languages''. We could also try to find a term that is more succinct than language family-specific models; for instance maybe genealogical models or models for genetically related languages. }
\section{Where are we today?}
\subsection{Resources}
\subsubsection{Models}
IndicBERT, IndicBART, MuRIL
\subsubsection{Data}
IndicCorp, Samanantar
\subsubsection{Benchmarks}
GLUECoS, IndicGLUE
\subsection{Organisations}
AI4Bharat, MSRI, Google Research India -- initiatives like CHaII to not only engage the community to work on IN languages but also as a means to collect data.



\section{Where do we want to be?}
Here I was thinking we can highlight limitations of current models. This can serve as the motivation to build MuRIL. We can lay out the performance gaps that exist between English and Indian languages, and in general the disparity in performance amongst IN languages themselves. Eventually we want to build technologies that treat all languages equally. (Can bring in some economic stuff here of utility and fairness -- Graham's work with Prof. Antonios)
\section{How can we get there?}
We argue that building geography? or language-family? specific models is an ideal way to get close to what we want to achieve and we lay out several benefits of taking this path, backed by empirical evidence (Going from most obvious to least). \seb{We can probably talk about genetically related languages although I'm not sure if languages from different language families can also be said to be genetically related.}

\seb{I think it would also be worth having a figure here for illustration that shows the spectrum of monolingual/multilingual models for evaluation based on the number of languages covered, together with benefits and deficits: At one end of the graph, we have monolingual models, which cover a single language as well as bilingual models. At the other end, we have massively multilingual models covering around 100 languages. In the middle, we have language family-specific models, which strike a balance of achieving good performance with a smaller number of parameters and enabling positive transfer for a set of languages.}

\subsection{Benefits of multilinguality without the curse}
It is often argued that positive transfer (amongst related languages) and zero-shot transfer (to low-resource languages w/ unlabelled data) are the key benefits of building multilingual models. These steps have greatly benefited several of the under-resourced languages which were being ignored by the community up until that point. (Cite Santy's paper on graph of number of languages being used in A* conferences). However XLM-R shows that limited model capacity and negative transfer to high-resource languages is the curse of going multilingual and models built on 15-17 languages perform best. Empirically, here we can have one experiment that compares MuRIL (built on 17 languages), XLM-R / mBERT (built on 100+ languages) and monolingual models (for HI and another low-resource language)

\subsection{Think of a name? (Pre-training)}
Once established that building language-family specific models is the way to go (w/ the above experiment), we can show how we attempt to improve upon this model, laying out a general recipe/template for any community looking to build a language-family specific model. Literature on pre-trained multilingual models attests to the fact that pre-training data, tokenization techniques and model/architecture are three key factors affecting multilingual representation. Most multilingual models released today closely follow the BERT architecture (barring a few like RemBERT). While exploring architectural changes unique to multilingual models (example, having language-specific and shared parameters in your model -- like in a few works in multilingual NMT) is a promising direction, we believe that working on data (and (linguistically motivated?) tokenizers?) is more inclusive of the community and can enable one to encompass a diverse set of languages spoken by members from several strata of society irrespective of their technical backgrounds.Given our focus on language diversity and inclusion, working on this will be more impactful in the long run. Therefore with data and tokenization as our cornerstone, we prove how they can be best exploited to build the best possible multilingual model. 

\subsection{Pre-training: Data}
Going from toughest --> easiest sources to obtain, also highlighting the costs to invest in each with expected returns. We can probably make a nice table in the end with exact numbers and their deltas (cost v/s return -- eventually arriving at the best techniques for low-cost and high-returns. It will mostly not be deterministic and may vary geographically, but the more universal/generalizable it is, the better would be its utility.) (Need to decide what our baseline will be.)

\seb{One thing to keep in mind here in this section is whether any of the aspects we highlight are specific to genetically related languages or to what extent they are applicable when collecting data for 100s of languages. Given the focus of the paper, we should stress aspects that highlight similarities or enable sharing of information between similar languages.}

\subsubsection{Translated Data (High Cost, Low Return)} 
\textbf{Conclusion}: Choosing non-EN target languages for translated data in pre-training can come here. \\ \textbf{Caveat}: Very tough to obtain parallel data in training. NMT doesn't exist for many languages. Training on clean monolingual data for longer steps gives benefits of TLM. So even if community invests in building this, its not as impactful. \\

\seb{We should also mention alternative objectives using parallel data but highlight that it is still an open research direction how to use parallel data most effectively.}

\subsubsection{Phonemized / Transliterated / Unicode shift Data (High/Mid/Low Cost, Mid-High Return?)}
Experiments with phoneme data / transliterated data can come here. If this has to be widely applicable I will need to provide a stat that languages in geographical proximity will be phonetically similar? Intuitively, I feel this would be the case because of cultural influences -- but it will be better to confirm this with a statistic. \\ \textbf{Conclusion}: This one shows good gains. (especially for low-resource languages and complex tasks like QA). Is widely applicable. \\ \textbf{Caveat}: OS phonemizers are pretty bad so if community can invest in building good phonemizers that would be great (High Cost). Else transliterating to latin (try devanagari?) works too (Mid cost). Maybe just unicode shifting to a common script (very low quality transliteration) might help too (ask prof. pushpak about this). (Low Cost)

\seb{This would also be useful for speech or training NLP+speech models}

\subsubsection{Monolingual Data (Mid/Low? Cost, Mid Return)}
Quantity + Quality --> Wikipedia / CC comparison results? (link to daan's paper for quality estimate of several corpora). \\ \textbf{Conclusion}: Invest in collecting high quality monolingual data as a starting step? (XLM-R too is proof of the benefits of high quality monolingual data) \\ \textbf{Caveat}: Some languages do not have online resources, hard to collect, scrape, clean etc. -- but there are works like Shruti Rijhwani's OCR work on endangered languages, which can be used for this purpose.

\seb{Another direction that we could highlight here is the potential to collect speech data for such languages but mention that this is still a very new direction.}
    
\subsubsection{Bilingual Dictionaries (Low Cost, Mid/Low Return?)}
RelateLM work can come here and we can do a small experiment to corroborate their findings (can extend MuRIL to a new language using the relateLM technique) \\ \textbf{Conclusion}: Investing in creating a bilingual dictionary helps? \\ \textbf{Caveat}: Some languages like Gondi don't even have a written script (can highlight what MSRI has done for this language in the subsequent sections)

\subsection{Pre-training: Tokenization}
Going from word --> byte level tokenizers (cost and return scales are relative).
\subsubsection{Word-level Models (Low Cost, Low Return)}
This we can simply cite relevant literature. A lot of past works highlight the sub-optimalities of word-level tokenizers because of OOV issues. That is how sub-word tokenizers came about. \\
\textbf{Caveat}: Easy to build, highly sub-optimal because of OOV issues

\subsubsection{Sub-word Models (Low/High Cost, High Return)}
WPM and SPM are low-cost; supervised morphological analysers is an attractive proposal (high-cost). Can highlight the WPM and SPM results here. For IN, WPM is better, but a better understanding of why (maybe the algorithm is biased toward learning better representations of morphologically complex languages like IN?) is needed on my part. \\
\textbf{Caveat}: Not flexible enough to deal with complex morphology -- example, many sub-words in MuRIL are simply morphological variations of each other (give an example). Also, unequal splitting, example, low-resource languages are highly segmented as compared to their high-resource languages.

\subsubsection{Character/Byte Models (Mid/High Cost, Mid Return?)}
We can call out efforts being made toward token-free models (byte/character level) and evaluate the SOTA models out there for IN (CANINE / Charformer?). There's been work in NMT hinting towards a composition over character trigrams being most effective in translating morphologically rich languages. With its strided convolutions over characters, CANINE may have a similar effect and is worth exploring for Indian languages. (although I believe it is not at par w/ subword models yet but is an interesting space to watch out for because by parameterizing the learning of subwords, we may be able to capture complex morphological nuances.). \\
\textbf{Caveat}: Deviates from standard architectures, not there yet in terms of performance as compared to their sub-word counterparts.


\subsection{Think of a name here? (Fine-tuning)}
Experiments with zero-shot transfer using HI/TA >> EN? Iulia's paper shows that, universally, DE and RU are better for cross-lingual zero-shot transfer as compared to EN. They show that this happens because, based on URIEL features, RU and DE are, on average, closer to the target languages in XTREME. With a limited set of target languages, we have the liberty to make linguistically motivated choices in choosing what languages we want to label data for? 

\subsection{Think of a name here? (Evaluation)}
Results with pseudo-translated test sets highlight that it is imperative to invest in creating evaluation benchmarks for the lower-resourced languages and for complex tasks like QA. Community engagement can be a way forward here. (highlight works of MSR-I like Karya, Gondi etc.). Building assistive interfaces for people to annotate data for their language is another possibility.

\subsection{Ethical Considerations}
Building language-family specific models is great but we must be wary of the biases they may exhibit over multilingual models built on data from a diverse set of languages. For example, MuRIL has a higher bias towards Indian names as compared to mBERT because it has been trained on Indian language data only. Therefore we must be wary of the context we use such models in


